Analysis of Timed and Long-Run Objectives for Markov Automata

Markov automata (MAs) extend labelled transition systems with random delays and probabilistic branching. Action-labelled transitions are instantaneous and yield a distribution over states, whereas timed transitions impose a random delay governed by an exponential distribution. MAs are thus a nondeterministic variation of continuous-time Markov chains. MAs are compositional and are used to provide a semantics for engineering frameworks such as (dynamic) fault trees, (generalised) stochastic Petri nets, and the Architecture Analysis & Design Language (AADL). This paper considers the quantitative analysis of MAs. We consider three objectives: expected time, long-run average, and timed (interval) reachability. Expected time objectives focus on determining the minimal (or maximal) expected time to reach a set of states. Long-run objectives determine the fraction of time to be in a set of states when considering an infinite time horizon. Timed reachability objectives are about computing the probability to reach a set of states within a given time interval. This paper presents the foundations and details of the algorithms and their correctness proofs. We report on several case studies conducted using a prototypical tool implementation of the algorithms, driven by the MAPA modelling language for efficiently generating MAs.

==> arrowSupport.tex <==
% ARROWS (from Arend)
\newcommand{\linefill}{%
    \cleaders
    \hbox{$\smash{\mkern-2mu\mathord-\mkern-2mu}$}%
    \hfill
    \vphantom{\lower1pt\hbox{$\rightarrow$}}%
}
\newcommand{\Ignore}[1]{}
\newcommand{\xleftnoend}[1][]{\mathrel-_{\vphantom{#1}}\mkern-11mu}
\newcommand{\xmid}[2][]{\stackrel{#2}{\linefill_{\vphantom{#1}}}}
\newcommand{\xrightArrow}[1][]{\mkern-11mu\rightarrow_{#1}}
\newcommand{\xmake}[1]{\mathrel{\lower0pt\hbox{$#1$}}}
\renewcommand{\xrightarrow}[2][]{\xmake{\xleftnoend[\smash{#1}]\xmid[\smash{#1}]{#2}\xrightArrow[#1]}}%

